Four Formal Models of IEEE 1394 Link Layer

We revisit the IEEE 1394 high-performance serial bus ("FireWire"), which became a success story in formal methods after three PhD students, by using process algebra and model checking, detected a deadlock error in this IEEE standard. We present four formal models for the asynchronous mode of the Link Layer of IEEE 1394: the original model in muCRL, a simplified model in mCRL2, a revised model in LOTOS, and a novel model in LNT.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{F. Lang, M. Volk (Eds):\\
Models for Formal Analysis of Real Systems (MARS 2024)\\
EPTCS 399, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.399.5}{10.4204/EPTCS.399.5}}
\pdfoutput=1

